Equivariant Algebraic Index Theorem

We prove a {\Gamma}-equivariant version of the algebraic index theorem, where {\Gamma} is a discrete group of automorphisms of a formal deformation of a symplectic manifold. The particular cases of this result are the algebraic version of the transversal index theorem related to the theorem of A. Connes and H. Moscovici for hypoelliptic operators and the index theorem for the extension of the algebra of pseudodifferential operators by a group of diffeomorphisms of the underlying manifold due to A. Savin, B. Sternin, E. Schrohe and D. Perrot.

==> inputactonqdef.tex <==
\RequirePackage{stmaryrd}
%Theorem Styles

\newtheoremstyle{theoremstyle}
  {10pt}      %  Space above
  {5pt}       %  Space below
  {\itshape}  %  Body font
  {}          %  Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries} %  Thm head font
  {:}         %  Punctuation after thm head
  {.5em}      %  Space after thm head: " " = normal interword space;
              %  \newline = linebreak
  {}          %  Thm head spec (can be left empty, meaning `normal')

\newtheoremstyle{examplestyle}
  {10pt}      %  Space above
  {5pt}       %  Space below
  {}          %  Body font
  {}          %  Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries} %  Thm head font
  {:}         %  Punctuation after thm head
  {.5em}      %  Space after thm head: " " = normal interword space;
              %  \newline = linebreak
  {}          %  Thm head spec (can be left empty, meaning `normal')

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}

\theoremstyle{definition}
\newtheorem{principle}[theorem]{Principle}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{notation}[theorem]{Notation}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%New Commands

%mboxes

\newcommand{\Log}{\mbox{Log}\hspace{0.1cm}}
\newcommand{\Id}{\mbox{Id}}
\newcommand{\Ids}{\mbox{\scriptsize Id}}
\newcommand{\Ad}{\mbox{Ad}\hspace{0.1cm}}
\newcommand{\ad}{\mbox{ad}\hspace{0.1cm}}
\newcommand{\ch}{\mbox{ch}\hspace{0.1cm}}
\newcommand{\Td}{\mbox{Td}}
\DeclareMathOperator*{\Tr}{\mbox{Tr}}
\newcommand{\Dim}{\mbox{Dim\hspace{0.1cm}}}

\newcommand{\Hom}{{\textrm{Hom}}}
\DeclareMathOperator*{\End}{\mbox{End}}
\newcommand{\Aut}{\mbox{Aut}}
\newcommand{\Inn}{\mbox{Inn}}
\DeclareMathOperator*{\Der}{\mbox{Der}}
\newcommand{\Coder}{\mbox{Coder}}
\newcommand{\Loc}{\mbox{Loc}}
\newcommand{\Symp}{\mbox{Symp}}
\newcommand{\Ext}{\mbox{Ext}}
\newcommand{\Tor}{\mbox{Tor}}

\DeclareMathOperator*{\Coker}{\mbox{Coker}}
\DeclareMathOperator*{\Ker}{\mbox{Ker}}

\newcommand{\Ima}{\mbox{Im}\hspace{0.1cm}}
\newcommand{\Ind}{\mbox{Ind\hspace{0.1cm}}}

\newcommand{\Fin}{\bf{Fin}}
\newcommand{\Bij}{\bf{Bij}}
\newcommand{\Gr}{\mbox{\scriptsize Gr}}
\newcommand{\Def}{\mbox{Def}}

\newcommand{\Sp}{\mbox{Sp}}
\newcommand{\Sps}{\mbox{\scriptsize Sp}}
\newcommand{\GL}{\mbox{GL}}
\newcommand{\GLs}{\mbox{\scriptsize GL}}
\newcommand{\Op}{\mbox{Op}}
\newcommand{\Ops}{\mbox{\scriptsize Op}}
\newcommand{\Diff}{\mbox{Diff}}

\newcommand{\dR}{\mbox{\tiny dR}}
\newcommand{\sbullet}{{\scriptscriptstyle\bullet}}

\newcommand{\Tot}{\mbox{Tot}}
\newcommand{\CH}{\mbox{H}}
\newcommand{\CHs}{\mbox{\scriptsize H}}
\newcommand{\CL}{\mbox{L}}
\newcommand{\K}{\mbox{K}}
\newcommand{\HC}{\mbox{HC}}
\newcommand{\chec}{\check{\mathrm{H}}}

%mathcals

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\cH}{\mathcal{H}}

\newcommand{\G}{{\mathcal{G}_\nabla}}
\newcommand{\TF}{\mathcal{T}_\mathcal{F}}
\newcommand{\GZ}{{\overline{\mathcal{G}_\nabla}}}
\newcommand{\FM}{{\mathcal{F}_M}}

%mathbbs

\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Nz}{\mathbb{N}\cup\{0\}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Cht}{\C\hhbar^\times}
\newcommand{\Ch}{\C\hhbar}
\newcommand{\T}{\mathbb{T}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\tLL}{\widetilde{\mathbb{L}}}

\newcommand{\sym}{\mathbb{S}}
\newcommand{\Ga}{\mathbb{F}}

\newcommand{\A}{\mathbb{A}}
\newcommand{\hO}{\hat{\mathbb{A}}}
\newcommand{\AH}{{\mathcal{A}^\hbar}}
\newcommand{\AHc}{{\mathcal{A}^\hbar_c}}
\newcommand{\AHl}{{\mathbb{A}_{(\hbar)}}}
\newcommand{\AW}{{\hat{\mathbb{A}}^\hbar}}
\newcommand{\AWl}{{\hat{\mathbb{A}}^{(\hbar)}}}
\newcommand{\AG}{\AH(M)\rtimes \Gamma}
\newcommand{\AGl}{\AHl\rtimes \Gamma}

\newcommand{\WW}{\mathbb{W}}
\newcommand{\WWH}{\mathbb{W}_{\hbar}}
\newcommand{\WWHl}{\mathbb{W}_{(\hbar)}}
\newcommand{\WWb}{\overline{\mathbb{W}}}

%mathfraks


\newcommand{\la}{\mathfrak{a}}
\newcommand{\gm}{\g_{\mathfrak{m}}}
\newcommand{\g}{\mathfrak{g}}
\newcommand{\tg}{\tilde{\mathfrak{g}}}
\newcommand{\lsp}{\mathfrak{sp}}

%shortcuts

\newcommand{\s}{\sigma}
\newcommand{\spx}{\triangle}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\hhbar}{\llbracket \hbar\rrbracket}
\newcommand{\hhhbar}{[\hbar^{-1},\hbar\rrbracket}

\newcommand{\umega}{\bar{\omega}}
\newcommand{\tdH}{\tilde{\mu}_\hbar}
\newcommand{\td}{\mu_\hbar}
\newcommand{\ftt}{\hat{\tau}_t}
\newcommand{\fta}{\hat{\tau}_a}
\newcommand{\ftaH}{\hat{\tilde{\tau}}_a}
\newcommand{\TT}{\tau_t}
\newcommand{\TA}{\tau_a}

%tildeshats

\newcommand{\tG}{\widehat{G}}
\newcommand{\tGr}{\widehat{G}_r}
\newcommand{\tM}{\widetilde{M}}
\newcommand{\tMr}{\widetilde{M}_r}
\newcommand{\tnabla}{\tilde{\nabla}}

%arrows

\newcommand{\inj}{\hookrightarrow}
\newcommand{\surj}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}

%moperators

\DeclareMathOperator*{\simK}{\sim}
\DeclareMathOperator*{\rightarrowm}{\rightarrow}
\DeclareMathOperator*{\leftarrowm}{\leftarrow}
\DeclareMathOperator*{\bigstarm}{\bigstar}

%constructions

\newcommand{\largewedge}[1]{\mbox{\Large $\wedge$}^{\hspace{-0.1cm}#1}\hspace{0.07cm}}
\newcommand{\tens}[1]{%
\mathbin{\mathop{\otimes}\limits_{#1}}%
}
\newcommand{\bigslant}[2]{{\ensuremath\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}


%options

\mathchardef\mhyphen="2D
\renewcommand{\phi}{\varphi}















